Regularization in Spider-Style Strategy Discovery and Schedule Construction

To achieve the best performance, automatic theorem provers often rely on schedules of diverse proving strategies to be tried out (either sequentially or in parallel) on a given problem. In this paper, we report on a large-scale experiment with discovering strategies for the Vampire prover, targeting the FOF fragment of the TPTP library and constructing a schedule for it, based on the ideas of Andrei Voronkov's system Spider. We examine the process from various angles, discuss the difficulty (or ease) of obtaining a strong Vampire schedule for the CASC competition, and establish how well a schedule can be expected to generalize to unseen problems and what factors influence this property.

==> tex/acknowledgments.tex <==
This work was supported by
the Czech Science Foundation project no.~20-06390Y (JUNIOR grant),
the European Regional Development Fund under the Czech project AI\&Reasoning no.~ CZ.02.1.01/0.0/0.0/15\_003/00004,
the project RICAIP no.~857306 under the EU-H2020 programme,
and
the Grant Agency of the Czech Technical University in Prague, grant
no.~SGS20/215/OHK3/3T/37.
\todo[inline]{Are these acknowledgments correct?}


==> tex/architecture.tex <==
% !TEX root = ../lncs.tex

\subsection{Overview}

Our process of constructing a strong schedule for Vampire on a given training problem set consisted of four phases.
Before giving a detailed description, we present an overview of the whole process:

\paragraph{Strategy discovery.}
\todo[inline]{TBA}

%\paragraph{Strategy and problem sampling.}
%First, strategies were sampled from a fixed distribution on the strategy space.
%Each sampled strategy was evaluated on one problem from the training set.
%The problems were sampled adaptively to concentrate on hard problems.
%
%\paragraph{Strategy selection.}
%The empirical hardness of the problems was assessed by counting successful and unsuccessful proof attempts observed so far.
%When a strategy solved a problem that was considered hard, the strategy was selected for simplification.
%The problem was stored along the strategy
%as a witness of the usefulness of the strategy.
%
%\paragraph{Strategy simplification.}
%Each selected strategy was simplified by local steps toward the default strategy.
%A step was taken as long as the performance on the witness problem did not deteriorate significantly.

\paragraph{Schedule optimization.}
Each minimized strategy was evaluated on each training problem.
The results of such evaluations were then used to construct a strategy schedule
that approximately optimizes empirical performance on the training problem set.

\todo[inline]{Create a picture or diagram of the whole pipeline.}

\begin{algorithm}
\caption{Schedule finder (high-level)}
\begin{algorithmic}[1]
% MaLeS uses $\mathfrak{S}$ to denote the set of "preselected strategies".
\State $\mathfrak{S} \gets \{\}$ \Comment{Strategy portfolio}
\Repeat
% Consider using \Configuration and \Instance instead of s and p.
\State $s, p, t \gets \Call{GetCandidateStrategy}$ \Comment{Strategy $s$, problem $p$, time $t$}
\State $s' \gets \Call{ImproveStrategy}{s, p, t}$
\State $\mathfrak{S} \gets \mathfrak{S} \cup \{s'\}$
\Until Time runs out \\
\Return $\Call{FitSchedule}{\mathfrak{S}}$
\end{algorithmic}
\end{algorithm}

\subsection{Target algorithm}

\subsubsection{Strategy space and distribution}

% Source of statistics about the strategy space:
% /home/filip/projects/strategizer/outputs/2022-10-18/10-18-12/cs/hyperparameters.csv

In our experiments, we used Vampire 4.7 as the target algorithm $\Algorithm$.
We selected 105 of its options as relevant for strategy optimization.\todo{Consider detailing the selection criteria.}\todo{Publish a list and reference it here. Consider including it in an appendix.}
To allow an efficient representation of the strategy distribution we wanted to sample,
we introduced several auxiliary parameters.
The strategy space was ultimately defined on 119 parameters
(92 categorical, 14 integer, and 13 floating point).

Not all combinations of the parameter values are valid configurations.
For example, the Vampire option \option{split\_at\_activation} only makes sense if the option \option{avatar} is set to the value \option{on};
the combination \option{avatar != on} and \option{split\_at\_activation != off} is considered invalid.
By excluding\todo{Not all excluding approaches are efficient. Explain.} the invalid parameter value combinations from the strategy space,
we make the strategy sampling and optimization more efficient.\todo{Explain.}
The distribution attributes the probability 0 to all invalid combinations of parameter values
and a nonzero probability to all the valid combinations of parameter values (i.e., strategies).

\todo[inline]{Explain how and why we avoided forbidden clauses.}
\todo[inline]{Consider describing the compromises we made -- simplification of the queue parameters.}
\todo[inline]{Describe how ratios are sampled and represented.}
\todo[inline]{Did we specialize for divisions?}

To concentrate on relatively strong strategies,
we used our domain knowledge to bias the distribution of some of the parameters.
\todo[inline]{Finish. Mention all expert knowledge: log vs. uniform, ...}

% Sampling:
% Email from FB to MS 2022-06-20
% nohup python -m strategizer cutoff.ub=500000 samples_per_iteration=1000 parallel.n_jobs=32 runs_dir=runs/universal_horizon_uns instances.list=data/universal_horizon_problems.txt time_limits=data/universal_horizon.txt instances.patterns=null hydra.verbose=__main__ &> stdout/universal_horizon_uns.txt &
% Stdout: /nfs/bartefil/git/strategizer/stdout/universal_horizon_uns.txt

\subsection{Training problem set}

\todo[inline]{Define $\InstancesTrain$. MS: Use a symbol without "train" in the name so that the reader does not expect a "test" set.}

\subsection{Strategy Discovery}
\label{sec:StrategyDiscovery}

See \cref{alg:discovery}.

\begin{algorithm}
\caption{Schedule finder procedures}
\label{alg:discovery}
\begin{algorithmic}[1]
\Require Target algorithm $\Algorithm$;
strategy space $\Configurations$;
instance set $\Instances$
\Ensure Strategy schedule $s$

% Actually, we run the sampling in batches to produce many candidate strategies.
\Procedure{GetCandidateStrategy}{}
% Sampling executions: https://docs.google.com/spreadsheets/d/1xSWEBFTL8DEALCa5wopL46VH8_KCK05veFvM5qo1U_M
% Example execution:
% Working directory: /nfs/bartefil/git/strategizer
% Stdout: stdout/strategizer-config-uniform.txt
% Output: outputs/2022-04-08/21-20-14
% Runs: runs/instances-ucb
% Cutoff: 10 s
% Configs and instances per iteration: 1000
% Instances: 14813
% Hyperparameters: 115
% Cost for timeout: 100 (?)
% Date started: 2022-04-08
% Script: strategizer/__main__.py
\Repeat
\State $\Configuration \gets$ random strategy sampled from $\Configurations$ (a fixed distribution)
\State $\Instance \gets$ problem from $\Instances$ that maximizes the \acrshort{ucb} of empirical hardness
% In the initial sampling, no time limits were provided. The limits were provided in later samplings.
\State $t \gets$ time of the best solution of $\Instance$ observed so far
% TODO: Disambiguate t.
\Until Vampire solves $p$ using $s$ in time $t$ \\
% TODO: Nest "return" under "procedure".
\Return $s, p, t$
\EndProcedure

\Procedure{ImproveStrategy}{s, p, t}
\Repeat
\State 
\Until
\EndProcedure

\end{algorithmic}
\end{algorithm}

\subsubsection{Strategy, problem, and time limit sampling}

We sampled strategies from a fixed distribution on $\Configurations$.
The distribution captured some intuition about the usefulness of some of the parameter values.\todo{Was the distribution actually fitted automatically?}
For example, the non-default values of the option \option{equality\_proxy} preprocess the input problem by replacing the equality with a fresh predicate $E$.
The semantics of $E$ are specified by including one or more axioms of reflexivity, symmetry, transitivity, or congruence.
These transformations help to solve a problem only in rare cases.
For this reason, we sampled the default value of the option 5 times as often as any of the 4 non-default values.

Each sampled strategy was evaluated on one problem from $\InstancesTrain$.
\todo[inline]{TBA}

\todo[inline]{Describe how the time limit (instruction limit) was sampled.}
\todo[inline]{MS: I provided horizon: the best time at which I already solve a given problem.}

Every time a sampled strategy solved a candidate problem,
this strategy was selected for simplification.

\subsubsection{Strategy simplification}

For each candidate strategy $s_0$,
we had a witness problem $p$ that was empirically hard and solvable by $s_0$.
\todo[inline]{Describe the simplification process.}
\todo[inline]{MS ran hillclimb on non-default options.

In each "round", a random permutation of options is taken and "minimized" -- defaulted if does not decrease performance.

"retrying luck" between rounds, the observations are discarded and EP is re-measured for the incumbent.

Each type has a different optimizer:
- categorical
- ordinal
- numeric - converted to ordinal
- ratio - shortening the decadic formatted expression

"precision cone" - set of values I am willing to switch to from an ugly number

Float: remove the least significant digit, allow both upper and lower bound.

Switch to better performance, or same performance and "more general"

Only at most 10 rounds are performed.

Sometimes, internal instruction limit is decreased as long as the solution probability is above 0.5.
}
\todo[inline]{Future work: full-fledged local search.}
\todo[inline]{Goal: greater interpretability and regularization (?).}



==> tex/greedy.tex <==
% !TEX root = ../jar.tex

\subsection{Success probability estimation}
\label{sec:SuccessProbabilityEstimation}

In this work, we assume that the target algorithm $\Algorithm$ is, in general, nondeterministic,
i.e., executing it multiple times with the same strategy, problem, and time limit may yield different results.
To accommodate the nondeterminism in the process of schedule optimization,
we define an empirical\todo{This means data-based. Is this clear?} estimate of the probability of success\todo{Success means solving the problem. Is this clear?} of an execution.
%The estimated probability of success maps a probability to every time $\Time$ and is based on a collection of empirical evaluations.

\subsubsection{Single observation}

%Let $\ProblemsTrain$ be a set of problem instances.
%Let $\StrategiesTrain$ be a set of strategies.
%For every problem $\Problem \in \ProblemsTrain$ and strategy $\Strategy \in \StrategiesTrain$,
Let us assume an arbitrary combination of a problem $\Problem$ and a strategy $\Strategy$.
A result of an evaluation\todo{Here we implicitly switch from \enquote{execution} to \enquote{evaluation}.} of $\AlgorithmInstance{\Strategy}$ on $\Problem$ with an arbitrary time limit is an observation $(\Status, \Time)$,
%Let $E_{\Problem, \Strategy} = \{(\Status_1, \Time_1), \ldots, (\Status_n, \Time_n)\}$ be a multiset of evaluations of $\AlgorithmInstance{\Strategy}$ on $\Problem$,
where $\Time$ is the runtime of the evaluation,
and $\Status \in \{\Success, \Fail, \Timeout\}$ is the final status of the evaluation:
\begin{itemize}
\item $\Success$ means that the evaluation solved $\Problem$ successfully,
for example, by deriving the empty clause in a refutational proof search.
If $\Algorithm$ was deterministic\todo{Is this counterfactual reasoning sufficiently clear? Alternatively, we could write about seeds.}, this would mean that $\Strategy$
reliably solves $\Problem$ when executed for at least $\Time$ time units and
fails to solve $\Problem$ when executed for a shorter time.
\item $\Fail$ means that the evaluation failed to solve $\Problem$ before reaching the time limit,
for example, by saturating the set of derived clauses using an incomplete strategy.
If $\Algorithm$ was deterministic, this would mean that $\Strategy$ fails to solve $\Problem$ irrespective of the time it is executed for.
\item $\Timeout$ means that the evaluation terminated prematurely due to a time limit.
%Specifically, had more time been allocated to the evaluation, it might eventually terminate with the status $\Success$ or $\Fail$.
If $\Algorithm$ was deterministic, this would mean that $\Strategy$ fails to solve $\Problem$ if executed for $\Time$ or fewer time units.
\end{itemize}

From one isolated observation $(\Status, \Time)$, we may estimate the result of a new execution with an arbitrary time limit $T$ by assuming that $\Algorithm$ is deterministic.
Specifically, we estimate that the new execution would successfully solve the problem if $T > \Time$ and $\Status = \Success$,
and that the new execution would fail if $T \leq \Time$ or $\Status = \Fail$.
In the remaining case ($T > \Time$ and $\Status = \Timeout$), we assume no knowledge about the result of the new execution.
\Cref{tab:status} summarizes the relation between the status $\Status$ and runtime $\Time$ observed in an evaluation, the time limit $T$ of a new execution, and the predicted success of the new execution.

\begin{table}
\centering
\caption{Estimated success of a new execution of an instantiated algorithm $\AlgorithmInstance{\Strategy}$ on a fixed problem $\Problem$ based on one evaluation result $(\Status, \Time)$}
\label{tab:status}
\begin{tabular}{@{}c|ccc@{}}
\toprule
New time limit $T$ & \multicolumn{3}{c}{Observed status $\Status$} \\
& $\Success$ & $\Fail$ & $\Timeout$ \\
\midrule
$T \leq \Time$ & No  & No & No \\
$T > \Time$ & Yes & No & Unknown \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Multiple observations}

\newcommand{\Observations}{E}
\newcommand{\ProbabilitySolve}[2]{P_\Success(#1 | #2)}

%Let $E_{\Problem, \Strategy} = \{(\Status_1, \Time_1), \ldots, (\Status_n, \Time_n)\}$
Let $\Observations = \{(\Status_1, \Time_1), \ldots, (\Status_n, \Time_n)\}$
be a multiset of observations of $\AlgorithmInstance{\Strategy}$ on $\Problem$.
From such a collection of evaluations, we estimate a probability of success of a new execution for an arbitrary time limit $T$:
$$
%\mli{successprob}(t') = \frac{\text{Number of observations $(s, t) \in E$ such that $s = \Success \land t < t'$}}{|\{(s, t) | (s, t) \in E \land (s \neq \Timeout \lor t \geq t')\}|}
\ProbabilitySolve{T}{E} = \frac
{\text{Number of observations $(\Status, \Time) \in \Observations$ such that $T > \Time \land \Status = \Success$}}
{\text{Number of observations $(\Status, \Time) \in \Observations$ such that $T \leq \Time \lor \Status \neq \Timeout$}}
$$
In other words, we divide the number of successful observations with runtime $< T$
by the number of all observations that reveal some information about the result of an execution with time limit $T$.\todo{Is this clear enough?}
\Cref{tab:success-probability-example} demonstrates the success probability estimation on an example collection of observations.

\begin{table}
\centering
\caption{Success probability estimate example}\label{tab:success-probability-example}
\begin{tabular}{@{}c|ccc|c@{}}
\toprule
Time & $\Success$ & $\Fail$ & $\Timeout$ & $P_\Success$ \\
\midrule
0 &   &   &   & 0/6 \\
1 &   &   & 1 & 0/6 \\
2 & 1 &   &   & 0/5 \\
3 &   &   & 1 & 1/5 \\
4 & 1 &   &   & 1/4 \\
5 & 1 &   &   & 2/4 \\
6 &   & 1 &   & 3/4 \\
7 &   &   &   & 3/4 \\
\bottomrule
\end{tabular}
\end{table}

%\subsubsection{Discussion}

%The schedule optimization algorithm allows using a different estimate of probability of success.
%For example, while our estimate is essentially frequentist, a Bayesian estimate might be used to bias the estimate towards a prior distribution.

\subsection{Set cover problem variants}

\todo[inline]{Remove or hide this section.}

\subsubsection{Set cover}

Input: Universe $U$, collection $S$ of sets whose union is $U$.

Output: Smallest sub-collection $C$ of $S$ whose union is $U$.

\subsubsection{Weighted set cover}

Input: $U$ and $S$ as in set cover, and a weight for each set in $S$.

Goal: Find a cover $C$ of $U$ that minimizes the total weight.

\subsubsection{Budgeted maximum coverage}

Input: Collection $\mathcal{S} = \{S_1, \ldots, S_m\}$ of sets with associated costs $c_i$, budget $L$.

Output: Subset $S'$ of $S$ such that the total cost of $S'$ does not exceed $L$ and the total weight of elements covered by $S'$ is maximized.

\subsubsection{Mapping to our task (deterministic version)}

U: Training problem set.

S: Set of actions (combinations of strategy and time). Each action covers all problems solved by the given strategy in the given time.

Cost of set is the time.

Weight of a problem is 1.

L: Time budget.

\subsection{Greedy algorithm}

We use a greedy algorithm to quickly find a strong strategy schedule using performance observations.
Our algorithm is based on an approximation algorithm for the budgeted maximum coverage problem \cite{DBLP:journals/ipl/KhullerMN99}.
In each iteration, our algorithm selects a slice (a combination of strategy and time) that maximizes the expected number of new problems solved per time unit and appends it to the schedule.

\newcommand{\TrainingSet}{\InstancesTrain}

Let $\TrainingSet$ be a training set of problems and $\StrategiesTrain$ be a training set of strategies.
For each $\Problem \in \TrainingSet$ and $\Strategy \in \StrategiesTrain$,
let $\Observations_{\Strategy, \Problem}$ be a multiset of training observations of evaluations of $\AlgorithmInstance{\Strategy}$ on $\Problem$.
Furthermore, let $\ProbabilitySolve{T}{E_{\Strategy, \Problem}}$ be an estimate of the probability that $\AlgorithmInstance{\Strategy}$ solves $\Problem$ when executed with time limit $T$, as described in \cref{sec:SuccessProbabilityEstimation}.

%\subsubsection{Budgeted maximum coverage}

%An instance of the budgeted maximum coverage problem consists of a collection $\mathcal{S} = \{S_1, \ldots, S_m\}$ of sets of elements of universe $X = \{x_1, \ldots, x_n\}$,
%set costs $\{c_i\}_{i=1}^m$,
%element weights $\{w_i\}_{i=1}^n$,
%and budget $L$.
%The goal is to find a collection of sets $\mathcal{S}' \subseteq \mathcal{S}$
%such that the total cost of sets in $\mathcal{S}'$ does not exceed budget $L$ (i.e., $\sum_{S_i \in \mathcal{S'}} c_i \leq L$)
%and the total weight of elements covered by $\mathcal{S}'$ is maximized.

%\subsubsection{Our algorithm}

Strategy schedule $\Schedule = [(\Strategy_1, T_1), \ldots, (\Strategy_n, T_n)]$ is a list of slices.
Slice $i$ specifies strategy $\Strategy_i$ to be executed and duration $T_i$ for which it is to be executed.
Note that in general, any given strategy may appear more than once in the schedule, and that the schedule specifies an order in which the slices are to be executed.

In each iteration of the schedule construction,
a slice is selected and appended to the schedule.
The slice is selected from a pool of candidate slices, which are extracted from the training observations:
$(\Strategy, T+1)$ is a candidate slice if and only if there is a problem $\Problem \in \TrainingSet$ that is solved by $\Strategy$ in time $T$,
that is $(\Success, T) \in \Observations_{\Strategy, \Problem}$.\todo{Stress that we deliberately omit extensions that would increase the score only by overtaking a timeout.}

In each iteration, the candidate slice that maximizes score is selected.
The score of candidate slice $(\Strategy, T)$ is the expected number of new problems solved per time unit:
$$
\mli{score}(\Strategy, T) = \frac{\sum_{\Problem \in \InstancesTrain} \ProbabilitySolve{T}{E_{\Strategy, \Problem}} (1 - P_\mli{solved}(\Problem))}{T}
$$
$\ProbabilitySolve{T}{E_{\Strategy, \Problem}}$ is computed from the training observations as described in \cref{sec:SuccessProbabilityEstimation}.
$P_\mli{solved}(\Problem)$ is an estimated probability that the partially constructed schedule $\mathcal{S}$ solves problem $\Problem$:
$$
P_\mli{solved}(\Problem | \Schedule, \Observations_\Problem) = 1 - \prod_{(\Strategy, T) \in \Schedule} (1 - \ProbabilitySolve{T}{E_{\Strategy, \Problem}})
$$

The schedule satisfies the time budget $\Budget$ if $\sum_{1 \leq i \leq n} T_i \leq \Budget$.
We continue extending the schedule until no further extension is possible without surpassing the time budget.

\begin{algorithm}
\caption{Greedy schedule estimator}
\begin{algorithmic}[1]
% MaLeS uses $\mathfrak{S}$ to denote the set of "preselected strategies".
\State $A \gets$ initial set of actions
\Repeat
\State $a \gets$ action that maximizes problems solved per time
\State Update schedule
\State Update $A$
\Until $A = \emptyset$ \\
\Return Schedule
\end{algorithmic}
\end{algorithm}


==> tex/introduction.tex <==
% !TEX root = ../lncs.tex

%The Introduction section, of referenced text \cite{bib1} expands on the background of the work (some overlap with the Abstract is acceptable).
%The introduction should not include subheadings.

\Glspl{atp} such as Vampire \cite{DBLP:conf/cav/KovacsV13} typically expose many parameters that control the proof search.
In the context of automatic theorem proving,
each valid configuration of parameters of an \gls{atp} is called a \emph{strategy}.
% Also known as: configuration, heuristic
The performance of an \gls{atp} on an input problem often varies greatly depending on the chosen strategy.
When dealing with a heterogeneous input problem distribution such as \acrshort{tptp} \cite{Sutcliffe2017},
a large performance gain can be achieved by employing a diverse portfolio of strategies instead of just one strong strategy \cite{DBLP:conf/flairs/WolfL98}.
% > If both conditions are satisfied, then a competitive use of different strategies can be more successful than the best single strategy.
% > A convincing illustration of this fact is the unexpected success of the theorem prover Gandalf at the theorem prover competition [CASC-14] [...], which applies this method by time slicing different strategies.
By ordering the strategies in a portfolio and assigning each a time limit,
we obtain a \emph{strategy schedule}.

In this paper, we describe a procedure we applied to construct strategy schedules for the \gls{atp} Vampire for the \gls{casc-j11} \cite{DBLP:journals/aicom/SutcliffeD23}.\todo{De-emphasize CASC-J11. We actually used a quite different procedure.}
While the task of schedule optimization has been tackled both in the context of automatic theorem proving \cite{%
% With algorithm configuration
DBLP:journals/jar/KuhlweinU15,DBLP:conf/mkm/HoldenK21,%
% Without algorithm configuration
DBLP:conf/cade/Tammet98,DBLP:conf/tableaux/StenzW00,DBLP:conf/ictai/HulaMJ21,DBLP:conf/cade/ManglaHP22}
and in general \cite{DBLP:conf/aaai/XuHL10},
our solution is original in several aspects:

\begin{itemize}
    %\item We implemented a strategy space for the \gls{atp} Vampire that allows efficient sampling of valid strategies.
    \item We used a novel point-based method of collecting a set of mutually complementary strategies.
    \item We designed and evaluated a powerful greedy algorithm that constructs a strategy schedule from performance measurements.
    Starting off with a standard approximation algorithm for the budgeted maximum coverage problem,
    we customized it to the scheduling problem to improve its performance.
    %We reduce schedule optimization to the budgeted maximum coverage problem
    %and use a standard approximation algorithm for the budgeted maximum coverage problem \cite{DBLP:journals/ipl/KhullerMN99}\todo{MS: Cite Chvatal or Tarjan.}
    %with custom optimizations.
    % How is it custom? By allowing the extension of a time slice that was added before. This is specific to scheduling.
    \item We further enriched the greedy schedule optimizer with several regularization mechanisms to improve generalization to unseen problems.
\end{itemize}

% How do we use budgeted maximum coverage?
% S: collection of sets. Each set is a set of problems solved by strategy s in time t.
% Cost of set: time t.
% Weight of problem p: 1.
% Budget L: time limit B.

For many years, Vampire's schedules for \acrshort{casc} were constructed by Andrei Voronkov with the help of a tool called Spider \cite{Spider}.
While we believe the above two points\todo{Which of the points?} are indeed unique to our approach, some of its other aspects (e.g., the strategy simplification described below) could have been indirectly inspired by Spider through discussions with its author.

\todo[inline]{
History of algorithm configuration etc. ...
well established field...
ATP have their own specifics...
Gandalf...
}

Terminology: time slicing - \url{https://en.wikipedia.org/wiki/Preemption_(computing)#Time_slice}


==> tex/perfect.tex <==
We have a set of problems $P$ and a set of strategies $S$.
For some of the pairs $p, s \in P \times S$,
we have a runtime $t(p, s)$ of a successful solution of problem $p$ with strategy $s$.
We assume that the solver is deterministic, so for each combination of $p$ and $s$ we have at most one runtime $t(p, s)$.
Note that a missing value $t(p, s)$ for some pair $p, s$ may signify either failure to solve $p$ with $s$, or the lack of evaluation of this problem-strategy pair.
We assume that the runtimes are integers.

We encode the problem of finding an optimum schedule with time budget $T$ as follows:
\begin{itemize}
\item For each strategy $s \in S$, we have a variable $t_s$ that takes integer values in the range from 0 to $T$.
This variable represents the time allocated to $s$ by the schedule.
To ensure that the schedule fits within the budget,
we constrain the strategy runtimes by the constraint $\sum_{s \in S} t_s \leq T$.
\item For each pair $p, s$ for which $t(p, s)$ is known,
we have a Boolean variable $u_{p, s}$.
If this variable is true, then $s$ is run long enough by the schedule to solve $p$.
We encode this property by the conditional constraint $u_{p, s} \to t_s \geq t(p, s)$.
\item Finally, for each problem $p$, we have a variable $u_p$.
If $u_p$ is true, then the schedule solves $p$.
We encode this property by the conditional constraint $u_p \to \bigwedge_{s \in S} u_{p, s}$.
\end{itemize}

Each model of this set of constraints defines a schedule $\{(s, t_s) | s \in S\}$
that solves the problems $\{p \in P | u_p\}$ within the time budget $T$.
Note that due to how the constraints are defined, such schedule may solve other problems in $P$ as well.

To obtain a strong schedule, we optimize this constraint program by maximizing the number of solved problems -- $\sum_{p \in P} u_p$.


==> tex/preliminaries.tex <==
% !TEX root = ../lncs.tex

\paragraph{Solver.}
A solver is a computer program that takes an input problem and attempts to solve it.
When the solver solves a problem, the user can extract the time taken by the attempt and, optionally,
additional information about the attempt or the solution.
If the solver is run with a time limit, the attempt may fail by running out of time.

For example, a \gls{fol} \gls{atp} is a solver that takes a \gls{fol} problem as the input.
The output is a status, such as THM (when a refutational proof is found),
SAT (when the clausified problem is satisfiable),
or UNK (when the proof search terminates but the satisfiability of the problem cannot be established due to the incompleteness of the calculus used in the proof search).

\paragraph{Automatic theorem prover.}
\todo[inline]{TBA}

\paragraph{Strategy.}
A strategy is a mapping that assigns a value to each parameter of the \gls{atp}.

%While the term \enquote{configuration} is common in literature about general configuration optimization,
%we use the term \enquote{strategy} that is common in the \gls{atp} community.
%Similarly, we use \enquote{strategy space} instead of \enquote{\acrlong{pcs}}\todo{Is \gls{pcs} worth mentioning?}.

\subsection{Instruction limiting}

\todo[inline]{Describe instruction limiting.}


==> tex/schedconstruction.tex <==
% !TEX root = ../lncs.tex

%This section describes several methods of constructing a strategy schedule using measurements generated by our strategy discovery procedure (see \cref{sect:discover}).
%The task is, assuming a fixed problems set $P$ and given a time budget $T$ specified in megainstructions,\todo{MS: ``megainstructions'' is a mouthful. I don't think we need to repeat it anymore. Just when talking about a concrete Mi value, but otherwise it's a time limit.}
%to generate a schedule $[(s_1, t_1), \ldots, (s_n, t_n)]$\todo{MS: Preliminaries introduce a sequence $S=(s_i,t_i)_{i=1}^n$, do we need a list?} that, given a new problem $p$ from the same distribution\todo{Can we avoid the concept of distribution? MS: Yes, please!} as $P$,
%is as likely as possible to solve $p$ in $T$ megainstructions.

%\subsection{Training Data}
%
%We assume that a target problem set $P$ is known upfront.
%From the strategy discovery procedure executed on $P$ (see \cref{sect:discover}),
%we obtain a set of optimized strategies $S$.
%Each of the strategies $s \in S$ has a witness problem $p_s$ and a time limit $T_s$\todo{Ensure the symbols $p_s$ and $T_s$ are defined in a previous section.}.
%Finally, since each strategy $s \in S$ has been evaluated on all problems in $P$ with the time limit $T_s$ (see \cref{sect:StrategyEvaluation}),
%we also know the solution times of all the combinations of in $S \times P$.
%These solution times are captured in the mapping $\SolveTime : S \times P \to \Nat \cup \{\infty\}$,\todo{MS: could we work with something shorter than $\SolveTime$? Co proste neco jako $E^s_p$?}
%where the value $\infty$ signifies a failure to solve the problem in the allocated time.
%
%We assume that Vampire is deterministic.\todo{MS: toho je divna veta. Vampire bude je nebo neni deterministic a bylo by divny, pokud bychom to nevedeli. Nechcem proste rict, ze ty data, co jsem namerili, povazujem za "gold" a dal uz neresime, ze tam mohla byt nepresnost mereni?}
%Our empirical assessment revealed that the runtimes of two evaluations of a strategy on a problem differ by not more than \Mi{10} in more than \SI{99.9}{\percent} cases.\todo{FB: I actually determined the difference by looking at how much the reported time overshoots the limit in timeouts.}
%To compensate for this noise in time measurement, we add a slack time of \Mi{10} to each slice of the final schedule.\todo{MS: tohle opravdu delas i v regularizacnich experimentech? Kazdopadne bych tady o ``empirical assessment'' vubec nemluvil.}
%\todo[inline]{Explain that the slack is negligible, unless it is not.}


\subsection{Greedy Schedule Construction}
\label{sec:greedy}

In this section, we introduce a greedy algorithm for schedule optimization.
The algorithm is derived from an approximation algorithm for the budgeted maximum coverage problem \cite{DBLP:journals/ipl/KhullerMN99}.\todo{Consider relating our problem and algorithm to budgeted maximum coverage in more detail.}\todo{Cite Chvatal here.}
We customize this general algorithm with several optimizations and regularizations specific for the problem of schedule construction.

The algorithm constructs the schedule iteratively.
In the base\todo{FB: I believe here we use \enquote{base} for the first time. Ensure consistency.} version of the algorithm, in each iteration, we choose strategy $s$ and time $t$ that maximize
the number of new problem solved per time unit,
and append the slice $(s, t)$ to the schedule;
see \cref{alg:greedy}.
The algorithm is polynomial in the sizes of the input problem set $P_\mli{train}$ and strategy set $S_\mli{train}$.

\begin{algorithm}
\caption{Greedy schedule construction (base version)}
\label{alg:greedy}
\begin{algorithmic}[1]
\Require Problems $P_\mli{train}$, strategies $S_\mli{train}$, solution times $\SolveTime$, time budget $T$
\Ensure Schedule $\Schedule$
\State $\Schedule \gets []$ \Comment{Schedule}
\State $P' \gets P_\mli{train}$ \Comment{Remaining problems to be solved}
\State $T' \gets T$ \Comment{Remaining budget}
\Repeat
\State $s, t \gets$ strategy $s$ and time $t$ that maximize the number of new problems solved per time:
$$\frac{|\{p \in P' | \SolveTimeP{s}{p} < t\}|}{t}$$
such that $t \leq T'$. \Comment{Stay within the budget}
\State $\Schedule \gets \Schedule + [(s, t)]$ \Comment{Extend the schedule}
\State $P' \gets \{p \in P' | \SolveTimeP{s}{p} \geq t\}$ \Comment{Remove the solved problems from $P'$}
\State $T' \gets T' - t$ \Comment{Update the remaining budget}
\Until No new problems can be solved. \\
\Return $\Schedule$
\end{algorithmic}
\end{algorithm}
%Time complexity of the algorithm without slice extensions: $O(|S| |P| (|S| + |P| \log |P|))$

\subsubsection{Slice Extension.}
\label{sec:SliceExtension}
To improve the performance of the resulting schedule,
in each iteration,
we allow extending one of the previously added slices
instead of adding a new one.
We follow the same criterion of maximizing the number of new problems solved per time.
Finally, to reduce the loss of anytime performance\todo{Discuss anytime performance somewhere before this.} of the output schedule,
we sort the schedule greedily using the same criterion as a post-processing step.\todo{Note that the same sorting can be used for an optimal schedule.}




==> tex/stochastic.tex <==
To optimize a schedule of a stochastic prover, we would need to maximize the expected number of problems solved:
$\sum_{p \in P} u_p$.
$u_p$ is a real-valued variable rather than a Boolean one.
More precisely, $u_p = 1 - \prod_{s \in S} (1 - u_{p, s})$,
where $u_{p, s}$ is the probability that strategy $s$ solves problem $p$.
We derive such probability from the data and $t_s$, the time assigned to $s$,
in the following manner:
$u_{p, s} = \max_{t \leq t_s} \mathrm{succ}(t, p, s) / \mathrm{fail}(t, p, s)$.

Optimum schedule for data $M$ on problems $P$ and strategies $S$:
Find $t$ that minimizes the expression
$$
\sum_{p \in P} \prod_{s \in S} \sum_{m \in M(p, s)} m_c \cdot [t_s \leq m_t]
$$
subject to $\sum_{s \in S} t_s \leq T$.

$t_s$ is the number of time units strategy $s$ is scheduled for.
$m_t$ is the time of observation $m$.

$m_c$ is the cost of failing to cover measurement $m$.
It expresses by how much the estimated probability of solving problem $p$ with strategy $s$ drops if strategy $s$ is scheduled for less than $m_t$ time units.

Alternative formulation of the objective (may be more suitable for Gurobi):
$$
\sum_{p \in P} \exp \sum_{s \in S} \log \sum_{m \in M(p, s)} m_c \cdot [t_s \leq m_t]
$$

$$
\sum_{p \in P} \exp \sum_{s \in S} \min_{m \in M(p, s)} \log m_f \cdot [t_s \leq m_t]
$$

$$
\sum_{p \in P} \exp \sum_{s \in S} \log \mathrm{failprob}(t_s, M(p, s))
$$

\todo[inline]{Describe how we determine failprob. Include a small tabular example: timeouts, successes, fail times.}
\todo[inline]{Describe greedy optimization. Actions at success time, not timeouts. See http://aitp-conference.org/2023/slides/FB.pdf}


==> tex/strategydistribution.tex <==
% !TEX root = ../jar.tex

In X\todo{Add a reference to a section.}, we described how we initially sampled strategies we used to attempt to solve hard problems.
We sampled the strategies from a hand-crafted distribution.
In this section, we describe how we could use the data we collected throughout our experiments to construct a strategy distribution that is more focused on solving hard problems.

We demonstrate the process on the \gls{fof} problem category.
Other problem categories can be approached analogously.

In total, we evaluated 2775 unique optimized strategies on all 8115 \gls{fof} training problems.
We denote the set of strategies by $\mathcal{S}$ and the set of problems by $P$.
Each of the strategies was evaluated only once on each problem\todo{Check if this is true.},
so we assume Vampire to be deterministic in this analysis.
Each of the strategies was evaluated with a fixed instruction limit between 2 to 535950 Mi\todo{How did we arrive at these limits?}.

Given a set of strategies $S \subseteq \mathcal{S}$ and a problem $p \in P$,
we consider $p$ uniquely solved by $S$ if some strategy $s \in S$ solves $p$,
and no strategy in $\mathcal{S} - S$ solves $p$.
In other words, by removing $S$ from $\mathcal{S}$, we would effectively lose all known solutions of $p$.

Let $S_\mathrm{av=on}$ ($|S_\mathrm{av=on}| = 2074$) be the set of all strategies in $\mathcal{S}$ with the AVATAR option enabled (denoted by \enquote{av=on}).
424 problems in $P$ are uniquely solved by $S_\mathrm{av=on}$.
We interpret these problems as the contribution from the option configuration \enquote{av=on}.
The 2074 strategies in $S_\mathrm{av=on}$ contributed 424 unique solved problems,
which is approximately \num{\fpeval{424/2074}} problems per strategy.

We consider the number of unique solved problems per strategy a measure of the utility of a given set of strategies.\todo{Justify. Describe the advantages of this measure.}
To derive a new sampling distribution for, e.g., the option AVATAR,
we calculate the number of unique solved problems per strategy for each of the choices of AVATAR (that is, \enquote{on} and \enquote{off}),
and normalize these numbers to a probability distribution.

Note that in strategies with the saturation algorithm FMB or InstGen,
AVATAR cannot be used at all.
These strategies are denoted by N/A in \cref{tab:av}
and they do not participate in the distribution.

\begin{table}
    \centering
    \caption{New distribution of the option AVATAR}\label{tab:av}
    \begin{tabular}{@{}l|rrrr@{}}
        \toprule
        Value & Strategies & \multicolumn{2}{c}{Unique problems} & Distribution \\
        && Absolute & Per strategy & \\
        \midrule
        off &  544 &  37 & 0.07 & 0.25 \\
        on  & 2074 & 424 & 0.20 & 0.75 \\
        N/A &  157 &   6 & 0.04 & \\
        \bottomrule
    \end{tabular}
\end{table}

\todo[inline]{---}

For example, the option AVATAR has two possible values: off and on.
Furthermore, the option is only enabled in configurations with the saturation algorithm Otter, LRS, and Discount, while it is disabled with the saturation algorithm FMB and InstGen.
Of the 2775 unique strategies we evaluated on all FOFUNS problems, ??? use the saturation algorithm FMB or InstGen,
and the remaining ???? use Otter, LRS, or Discount.

Let us assume an arbitrary problem $P$ in isolation.
The problem was evaluated using some of the 2775 strategies with some instruction limits.
% Should we only consider strategies that were evaluated on all problems?
% Should we only consider strategies that were evaluated with some minimum time limit? Should we fix a time limit?

\begin{table}
    \centering
    \caption{Saturation algorithm}\label{tab:sa}
    \begin{tabular}{@{}l|rrrr@{}}
        \toprule
        Value & Strategies & Unique problems & Unique per strategy & Normalized \\
        \midrule
        Otter    &  273 &  33 & 0.12 & 0.32 \\
        LRS      & 1493 & 154 & 0.10 & 0.27 \\
        Discount &  852 &  74 & 0.09 & 0.23 \\
        FMB      &   93 &   6 & 0.06 & 0.17 \\
        InstGen  &   64 &   0 & 0.00 & 0.00 \\
        \bottomrule
    \end{tabular}
\end{table}

We can use a similar approach to determine conditional sampling distributions.


\begin{table}
    \centering
    \caption{Sampling ratios of SAC depending on SA}\label{tab:sac-sa}
    \begin{tabular}{@{}l|rr@{}}
        \toprule
        SA & sac=off & sac=on \\
        \midrule
        Otter & 1.00 & 0.00 \\
        LRS & 0.68 & 0.32 \\
        Discount & 0.22 & 0.78 \\
        \midrule
        Unconditional & 0.61 & 0.39 \\
        \bottomrule
    \end{tabular}
\end{table}

\subsection{Issues}

We always assume a certain background distribution of strategies.
This distribution may be quite different from the distribution we use when sampling.

\todo[inline]{How could we do better? Perhaps by comparing the values of one option (e.g. av=off and av=on) on a fixed reasonable background strategy distribution.}


==> tex/task.tex <==
% !TEX root = ../lncs.tex

Let us assume that we have a parameterized target solver.
Furthermore, let us assume we have a target set of problems -- input instances for the target solver.

The main task is to find a strategy schedule -- a sequence of time slices, each of which consists of a strategy and a time limit.
We try to find a schedule that maximizes the expected number of solved problems in a given time budget.

\subsection{Specifics of ATP}
\todo[inline]{Ideally, we would say something like \enquote{We cannot use SMAC because we have too many instances.}.}
\paragraph{Large strategy space.}
The strategy space spans a large number of parameters.
For example, the Vampire strategy space we sampled consists of 118\todo{Really?} parameters.\todo{Compare to other benchmarks.}

\paragraph{Heterogeneous problem space.}
The strategy schedule is optimized on a large number of input problems.
For example, to optimize for the section \gls{fof} of CASC-J11,
we trained on 7866\todo{We would train on this many problems if we decided to train on the whole problem set.} problems.

Moreover, the problem set is diverse.\todo{Justify.}

\paragraph{Heavy-tailed solving time distribution.}
It is usually better to try many strategies with short time limits than few strategies with long time limits.
The resulting schedule is expected to have many short time slices and a few long time slices.

\todo[inline]{Specifics of our case:
- Many training instances
- Strategy schedule?
- If a solution exists, then a quick solution exists (Giles Reger: ...)
ATP is harder than SAT.
For this reason, it has the Giles' property,
and we want to restart proof searches with new configs often.
We want to have many short slices in the schedule.

Characteristic result: the schedule has many short slices and a few long slices.}

